Spectral Greedy Coresets for Graph Neural Networks

The ubiquity of large-scale graphs in node-classification tasks significantly hinders the real-world applications of Graph Neural Networks (GNNs). Node sampling, graph coarsening, and dataset condensation are effective strategies for enhancing data efficiency. However, owing to the interdependence of graph nodes, coreset selection, which selects subsets of the data examples, has not been successfully applied to speed up GNN training on large graphs, warranting special treatment. This paper studies graph coresets for GNNs and avoids the interdependence issue by selecting ego-graphs (i.e., neighborhood subgraphs around a node) based on their spectral embeddings. We decompose the coreset selection problem for GNNs into two phases: a coarse selection of widely spread ego graphs and a refined selection to diversify their topologies. We design a greedy algorithm that approximately optimizes both objectives. Our spectral greedy graph coreset (SGGC) scales to graphs with millions of nodes, obviates the need for model pre-training, and applies to low-homophily graphs. Extensive experiments on ten datasets demonstrate that SGGC outperforms other coreset methods by a wide margin, generalizes well across GNN architectures, and is much faster than graph condensation.

==> text/tf4-other.tex <==
% \begin{figure*}[t]
% \centering
%     \begin{subfigure}[b]{0.32\textwidth}
%     \includegraphics[width=.93\linewidth]{figs/fig-ego-compression.png}

%     \caption{\label{fig:ego-compression}Test accuracy versus the selected data size of selecting nodes and diffusion ego-grpahs with/without PCA-based compression of node attributes.}
%     \end{subfigure}
% \hfill
%     \begin{subfigure}[b]{0.32\textwidth}
%     \includegraphics[width=.99\linewidth,trim={5pt 5pt 5pt 5pt},clip]{figs/fig-ablation-homo.png}
%     \caption{\label{fig:ablation-homo}SGGC is more robust than SCGIGA on low-homophily graphs. We select the coresets on the edge-added graph with lower homophily, but train and test GCNs on the original graph.}
%     \end{subfigure}
% % \capbtabbox[0.32\textwidth]{%
% %     \adjustbox{max width=.99\linewidth}{%
% %     {\renewcommand{\arraystretch}{1.6}%
% %     {\Huge
% \hfill
%     \begin{subfigure}[b]{0.32\textwidth}
%         \adjustbox{max width=.99\linewidth}{%
%         {\renewcommand{\arraystretch}{1.6}%
%         {\Huge
% \begin{tabular}{ccccc} \toprule
%     \multirow{3}{*}{Method} & \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Architecture\\[-5pt]used during\\[-5pt]Compression\end{tabular}} & \multicolumn{3}{c}{\multirow{2}{*}{Downstream Architecture}}              \\
%                             &                                                                                                   & \multicolumn{3}{c}{}                                                                \\ \cmidrule(lr){3-5} 
%                             &                                                                                                   & GCN                       & SAGE                      & SGC                         \\ \midrule
%     \multirow{3}{*}{GCond}  & GCN                                                                                               & 70.6$\pm$3.7              & 60.2$\pm$1.9              & 68.7$\pm$5.4                \\
%                             & SAGE                                                                                              & 77.0$\pm$0.7              & 76.1$\pm$0.7              & \textbf{77.7$\pm$1.8}       \\
%                             & SGC                                                                                               & \textbf{80.1$\pm$0.6}     & \textbf{78.2$\pm$0.9}     & \textbf{79.3$\pm$0.7}       \\ \arrayrulecolor{black!50} \midrule
%     \textbf{SGGC (Ours)}    & N/A                                                                                               & \textbf{80.2$\pm$1.1}     & \textbf{79.1$\pm$0.7}     & \textbf{78.5$\pm$1.0}       \\ \bottomrule
%     \end{tabular}
%     %\vspace{10pt}
%     \caption{SGGC generalizes better across GNN architectures than graph condensation (GCond) on Cora with a 50\% ratio.}\label{tab:generalization}
% \end{subfigure}
% \end{figure*}


% \begin{figure*}[t]
% \centering
%     \begin{subfigure}[b]{0.32\textwidth}
%         \includegraphics[width=\linewidth]{figs/fig-ego-compression.png}
%         \caption{Test accuracy versus the selected data size of selecting nodes and diffusion ego-graphs with/without PCA-based compression of node attributes.}
%         \label{fig:ego-compression}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.32\textwidth}
%         \includegraphics[width=\linewidth,trim={5pt 5pt 5pt 5pt},clip]{figs/fig-ablation-homo.png}
%         \caption{SGGC is more robust than SCGIGA on low-homophily graphs. We select the coresets on the edge-added graph with lower homophily, but train and test GCNs on the original graph.}
%         \label{fig:ablation-homo}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.32\textwidth}
%     \centering
%     \adjustbox{max width=0.9\linewidth, max height=0.75\textheight, center}{% Adjust size and center
%     \begin{minipage}{\textwidth}
%     \renewcommand{\arraystretch}{1.2} % Adjust line spacing for appearance
%     \begin{tabular}{ccccc}
%         \toprule
%         Method & \begin{tabular}[c]{@{}c@{}}Architecture\\used during\\Compression\end{tabular} & GCN & SAGE & SGC \\
%         \midrule
%         GCond & GCN & 70.6$\pm$3.7 & 60.2$\pm$1.9 & 68.7$\pm$5.4 \\
%         & SAGE & 77.0$\pm$0.7 & 76.1$\pm$0.7 & \textbf{77.7$\pm$1.8} \\
%         & SGC & \textbf{80.1$\pm$0.6} & \textbf{78.2$\pm$0.9} & \textbf{79.3$\pm$0.7} \\
%         \textbf{SGGC (Ours)} & N/A & \textbf{80.2$\pm$1.1} & \textbf{79.1$\pm$0.7} & \textbf{78.5$\pm$1.0} \\
%         \bottomrule
%     \end{tabular}
%     \end{minipage}
%     }
%     \caption{SGGC generalizes better across GNN architectures than graph condensation (GCond) on Cora with a 50\% ratio.}
%     \label{tab:generalization}
% \end{subfigure}
% \end{figure*}
